Provable Methods for Searching with an Imperfect Sensor

Assume that a target is known to be present at an unknown point among a finite set of locations in the plane. We search for it using a mobile robot that has imperfect sensing capabilities. It takes time for the robot to move between locations and search a location; we have a total time budget within which to conduct the search. We study the problem of computing a search path/strategy for the robot that maximizes the probability of detection of the target. Considering non-uniform travel times between points (e.g., based on the distance between them) is crucial for search and rescue applications; such problems have been investigated to a limited extent due to their inherent complexity. In this paper, we describe fast algorithms with performance guarantees for this search problem and some variants, complement them with complexity results, and perform experiments to observe their performance.

==> belief_updates.tex <==
\label{sec:belief_updates}
Consider an $s$-step schedule $\psi$ of an $(\bfalpha, \bfbeta)$-imperfect searcher. Given the erroneous detection random variables $(Y_{\psi(t)})^s_{t=1}$, how does the probability vector $(\p{i}{t})^n_{i=1}$ change over time? Specifically, can we compute the probability vector $(\p{i}{s})^n_{i=1}$ quickly and efficiently? In this section, we provide a simple algorithm (\Cref{belief updates algo}), based on the theoretical results we develop (\Cref{order does not matter main thm,belief probability main thm}), to compute this vector. Current methods use a recursive expression \cite{chung_decision-making_2007,chung_analysis_2012,yu_bayesian-based_2020} to compute this vector and therefore require $\Omega(ns)$-time for the computation. We show that this can be improved to $\order{n \log{s}}$-time. Bayesian beliefs updating is also of great independent interest and has been studied for multi-agent search (with perfect detection~\cite{bourgault2003coordinated}) as well as other information gathering problems~\cite{marchant2014bayesian,otte2021path}. Our approach is tailored for efficiency specific to our problem.

Our main contribution in this regard is \Cref{order does not matter main thm}, where we show that two (executions of) schedules that have the same \textit{characteristics} (defined below) produce the same probability vector on completion. This enables us to compute the final probability vector using an ``easier" schedule in \Cref{belief probability main thm}. The proofs of the claims that follow are routine (but the proof of \Cref{order does not matter mid} is slightly involved) applications of \textit{Bayes' Theorem} and mathematical induction and have been deferred to the supplementary material %Appendix -- see \Cref{updating beliefs appendix}. 
We define $\alphaC_i$ and $\betaC_i$ to be the complementary probabilities of $\alpha_i$ and $\beta_i$ respectively. 

\begin{lemma} \label{one-step update}
    Let $\psi(0) = \psi(1) = i$. Then,
    \begin{equation}\label{update when searcher says yes}
        \Pr{X = j \mid Y_{\psi(1)} = 1} = 
        \begin{cases}
            \displaystyle\frac{\betaC_ip_i}{\betaC_ip_i + \alpha_i(1 - p_i)} \text{ if }j = i\\
            \displaystyle\frac{\alpha_ip_j}{\betaC_ip_i + \alpha_i(1 - p_i)} \text{ if }j \neq i
        \end{cases}
    \end{equation}
    \begin{equation}\label{update when searcher says no}
        \Pr{X = j \mid Y_{\psi(1)} = 0} = 
        \begin{cases}
            \displaystyle\frac{\beta_i p_i}{\beta_i p_i + \alphaC_i(1-p_i)} \text{ if }j = i\\
            \displaystyle\frac{\alphaC_ip_j}{\beta_i p_i + \alphaC_i(1-p_i)} \text{ if }j \neq i
        \end{cases}
    \end{equation}
\end{lemma}
\begin{lemma}\label{order does not matter mid}
    Consider a schedule $\psi$ (with $s = |\psi| > 1$) and $1 \leq t_1 < t_2 \leq |\psi|$. Let $i = \psi(t_1)$ and $j = \psi(t_2)$. Construct a schedule $\psi'$ with $\psi'(t_1) = j$, $\psi'(t_2) = i$, and $\psi'(t) = \psi(t)$ for all $t \notin \{t_1,t_2\}$. If $(Y_{\psi(t_1)},Y_{\psi(t_2)}) = (Y_{\psi'(t_2)},Y_{\psi'(t_1)})$ and $Y_{\psi(t)} = Y_{\psi'(t)}$ for all other $t$, $\p[(\psi)]{k}{s} = \p[(\psi')]{k}{s}$ for all $1 \leq k \leq n$.
\end{lemma}

Consider an execution of a schedule $\psi$. We let $a_i(\psi)$ and $b_i(\psi)$ (we drop the parenthesis when appropriate) be the number of times that $\psi$ searches $v_i \in V$ and returns 1 and 0 respectively -- i.e.,
\begin{equation}\label{a_i and b_i}
    \begin{split}
        a_i(\psi) &= |\{t \mid \psi(t) = i \  \land \  Y_{\psi(t)} = 1\}|\\
        b_i(\psi) &= |\{t \mid \psi(t) = i \  \land \  Y_{\psi(t)} = 0\}|
    \end{split}
\end{equation}

We say that two (executions of) schedules $\psi$ and $\psi'$ have the same \textit{characteristics} if $a_i(\psi) = a_i(\psi')$ and $b_i(\psi) = b_i(\psi')$ for all $1 \leq i \leq n$. Note that the order in which these schedules visit points (or the order in which they erroneously detect the target at a point) does not have to be the same for two schedules to have the same characteristics. Our definition, however, implies that schedules having the same characteristics search a point the same number of times (since $a_i(\psi) + b_i(\psi)$ is the number of times that $\psi$ searches $v_i$) and therefore implies that $|\psi| = |\psi'|$. We now show, using the developed machinery, that if $\psi$ and $\psi'$ have the same characteristics, then the probability vector at the end of their executions is the same.    
\begin{theorem}\label{order does not matter main thm}
    Consider two (executions of) schedules $\psi$ and $\psi'$ with the same characteristics. Let $s = |\psi| = |\psi'|$. Then, $\p[(\psi)]{i}{s} = \p[(\psi')]{i}{s}$ for all $1 \leq i \leq n$.
\end{theorem}
\begin{proof}
    Note that both $\psi$ and $\psi'$ can be interpreted as permutations of the multiset $S$ containing $a_i(\psi) + b_i(\psi)$ copies of each $v_i \in V$. By \Cref{order does not matter mid}, all schedules that correspond to \textit{transpositions} (permutations that change the ordering of exactly two elements of $S$) on $S$ have the same probability of success. Since any permutation on $S$ can be expressed as a composition of transpositions \cite{stanton_listing_1986}, our claim follows. 
\end{proof}
The following lemma was also reported in \cite{kress_optimal_2008,chung_analysis_2012}, but we provide an alternate (and simpler) proof using \Cref{order does not matter main thm} in the supplementary document.
%Appendix (\Cref{updating beliefs appendix}). 
\begin{lemma}\label{repeated searching of one node}
    Let $\psi$ be a schedule that only searches one vertex $v_i \in V$. Let $|\psi| = s$ (so $s$ is the number of times it searches $v_i$). Then, 
    \[
        \p{j}{s} = 
        \begin{cases}
            \displaystyle\frac{\betaC_i^{a_i} \cdot \beta_i^{b_i}p_i}{\betaC_i^{a_i} \cdot \beta_i^{b_i}p_i + \alpha_i^{a_i} \cdot  \alphaC^{b_i}_i(1 - p_i)} \text{ if }j = i\\
            \displaystyle\frac{\alpha_i^{a_i} \cdot \alphaC_i^{b_i}p_j}{\betaC_i^{a_i} \cdot \beta_i^{b_i}p_i + \alpha_i^{a_i} \cdot  \alphaC^{b_i}_i(1 - p_i)} \text{ if }j \neq i
        \end{cases}
    \]
\end{lemma}

Using the previous two results, we can prove the main theorem in this section.
\begin{theorem}\label{belief probability main thm}
    Let $\psi$ be a schedule and $s = |\psi|$. Then, for $1 \leq i \leq n$, if $\alpha^*_i$ and $\beta^*_i$ denote $\alpha_i^{a_i} \cdot  \alphaC^{b_i}_i$ and $\betaC_i^{a_i} \cdot \beta_i^{b_i}$ respectively,
    \begin{equation}\label{belief probability}
        \p[(\psi)]{i}{s} = \frac{\prod_{j \neq i}\alpha^*_j \cdot \beta^*_ip_i}{\sum^n_{k=1}\left(\prod_{j \neq k}\alpha^*_j \cdot \beta^*_k p_k 
        \right)}
    \end{equation}
\end{theorem}
\begin{proof}
    To compute $\p[(\psi)]{i}{s}$, we consider the schedule $\psi'$ which searches $v_1$ $a_1 + b_1$ times, followed by $v_2$ $a_2 + b_2$ times, and so on. By \Cref{order does not matter main thm}, $\p[(\psi)]{i}{s} = \p[(\psi')]{i}{s}$. By repeated application of \Cref{repeated searching of one node} (consider each $(a_j + b_j)$-length search of $v_j$ a separate schedule and update the initial probabilities of the nodes for the next schedule), our result follows.
\end{proof}

As noted at the outset of this section, \Cref{belief probability main thm} enables us to compute the final probability vector in $\order{n\log{s}}$-time (an exponential improvement in $s$ over recursive methods in \cite{chung_decision-making_2007,chung_analysis_2012,yu_bayesian-based_2020}). The details are presented in \Cref{belief updates algo}.
%in the supplementary document. Appendix (\Cref{updating beliefs appendix}). 
This simple algorithm relies on \textit{repeated squaring} (see Chapter 31.6 in \cite{cormen_introduction_2009}) to facilitate the computation of each $\alpha^*_i$ and $\beta^*_i$ in $\order{\log{s}}$-time. This takes $\order{n\log{s}}$-time in total; the rest of the computations take only linear time.

\begin{algorithm}[ht]
    \caption{Computing Final Probability Vector}
    \label{belief updates algo}
    \KwData{$P_X$, $(\bfalpha, \bfbeta)$, and the characteristics $(a_i, b_i)^n_{i=1}$ of an execution of a schedule $\psi$}
    \KwResult{$\p[(\psi)]{i}{|\psi|}$}
    \While{$1 \leq i \leq n$}
    {
        \tcp{Use repeated squaring to in the function to compute exponents}
        $\alpha^*_i \gets \text{\textsc{ComputeExponent}}(\alpha_i,a_i) \cdot \text{\textsc{ComputeExponent}}(\alphaC_i,b_i)$\; \label{belief updates line 1}
        $\beta^*_i \gets \text{\textsc{ComputeExponent}}(\betaC_i,a_i) \cdot \text{\textsc{ComputeExponent}}(\beta_i,b_i)$\;\label{belief updates line 2}
    }
    $\alpha^* \gets \prod^n_{i = 1}\alpha^*_i$\;
    \tcp{$\p[(\psi)]{i}{|\psi|}$ initially denotes the probabilities before normalisation} 
    $\p[(\psi)]{i}{|\psi|} \gets \frac{\alpha^* \cdot \beta^*_i p_i}{\alpha^*_i}$ for each $1 \leq i \leq n$\;
    $d \gets \sum^n_{i=1}\p[(\psi)]{i}{|\psi|}$\;
    \tcp{Normalise with $d$}
    $\p[(\psi)]{i}{|\psi|} \gets \frac{\p[(\psi)]{i}{|\psi|}}{d}$ for each $1 \leq i \leq n$\;
    \Return{$(\p[(\psi)]{i}{|\psi|})^n_{i=1}$}
\end{algorithm}

We note that \Cref{belief probability} simplifies significantly when we do not have false positives -- i.e., $\alpha_i = 0$ for all $1 \leq i \leq n$. Therefore, if $Y_{\psi(t)} = 1$ for any $t$, then the probability that $X = \psi(t)$ becomes 1 while all other probabilities drop to 0. When $Y_{\psi(t)} = 0$ for all $t$, $a_i = 0$ for all $i$. With these two observations, we have, as in \cite{lossner_discrete_1982},  
\begin{equation}\label{belief probability one error}
        \p[(\psi)]{i}{s} = \frac{\beta^{b_i}_ip_i}{\sum^n_{j=1}\left(\beta^{b_i}_ip_i \right)}
\end{equation}
For consistency between \Cref{belief probability,belief probability one error} we assume that the $0^0$ terms (which appear in the computation of $\alpha^*_i$) are equal to 1. Moreover, note that $b_i$ represents the number of times that $\psi$ searches $v_i$ in \Cref{belief probability one error}. 

\subsection{Discussions from 
\Cref{updating beliefs}}\label{updating beliefs appendix}
\begin{proof}[Proof of \Cref{one-step update}]
    Using \textit{Bayes' Theorem}, 
    \begin{align*}
        \Pr{X = j \mid Y_{\psi(1)} = 1} &= \frac{\Pr{Y_{\psi(1)} = 1 \mid  X = j}\Pr{X = j}}{\Pr{Y_{\psi(1)}= 1}}\\
        &=\frac{\Pr{Y_{\psi(1)} = 1 \mid  X = j}\Pr{X = j}}{\Pr{Y_{\psi(1)}= 1 \mid X = i} \Pr{X = i} + \Pr{Y_{\psi(1)}= 1 \mid X \neq i} \Pr{X \neq i}}\\
        & = \frac{\Pr{Y_{\psi(1)} = 1 \mid  X = j}\Pr{X = j}}{\betaC_ip_i + \alpha_i(1 - p_i)}
    \end{align*}
    The last equality follows from \Cref{yes | present,yes | not present}. Applying these equations again to the cases $j = i$ and $j \neq i$ gives us \Cref{update when searcher says yes}.
    
    Similarly,
    \begin{align*}
        \Pr{X = j \mid Y_{\psi(1)} = 0} &= \frac{\Pr{Y_{\psi(1)} = 0 \mid  X = j}\Pr{X = j}}{\Pr{Y_{\psi(1)} = 0}}\\
        &=\frac{\Pr{Y_{\psi(1)} = 0 \mid  X = j}\Pr{X = j}}{\Pr{Y_{\psi(1)}= 0 \mid X = i} \Pr{X = i} + \Pr{Y_{\psi(1)}= 0 \mid X \neq i} \Pr{X \neq i}}\\
        & = \frac{\Pr{Y_{\psi(1)} = 0 \mid  X = j}\Pr{X = j}}{\beta_ip_i + \alphaC_i(1 - p_i)}
    \end{align*}
    The last equality follows from \Cref{no | present,no | not present}. Applying these equations again to the cases $j = i$ and $j \neq i$ gives us \Cref{update when searcher says no}.
\end{proof}

Before we prove \Cref{order does not matter mid}, we first prove the following lemma.

\begin{lemma}\label{two-step update}
    Consider a 2-step schedule $\psi$ and let $i = \psi(1)$ and $j = \psi(2)$. Construct a (2-step) schedule $\psi'$ with $\psi'(1) = j$, $\psi'(2) = i$. If $(Y_{\psi(1)},Y_{\psi(2)}) = (Y_{\psi'(2)},Y_{\psi'(1)})$, then $\p[(\psi)]{k}{2} = \p[(\psi')]{k}{2}$ for all $1 \leq k \leq n$.
\end{lemma}

\begin{proof}[Proof of \Cref{two-step update}]
    First, we compute this probability for $\psi$. We have four cases depending on the (two) values of $Y_{\psi(1)}$ and $Y_{\psi(2)}$. The probabilities $\p[(\psi)]{i}{2}$, $\p[(\psi)]{j}{2}$, and $\p[(\psi)]{k}{2}$ (for all $k \notin \{i,j\}$) can be obtained by applying \Cref{one-step update} twice. These probabilities are tabulated in \Cref{second updates}. The denominators of these probabilities are given below: 
    \begin{align*}
        d_{(0,0)} &= \beta_i\alphaC_j p_i + \alphaC_i\beta_jp_j + \alphaC_i \alphaC_j (1 - p_i - p_j)\\
        d_{(0,1)} &= \beta_i\alpha_j p_i + \alphaC_i\betaC_jp_j + \alphaC_i \alpha_j (1 - p_i - p_j)\\
        d_{(1,0)} &= \betaC_i\alphaC_j p_i + \alpha_i\beta_jp_j + \alpha_i \alphaC_j (1 - p_i - p_j)\\
        d_{(1,1)} &= \betaC_i\alpha_j p_i + \alpha_i\betaC_jp_j + \alpha_i \alpha_j (1 - p_i - p_j)
    \end{align*}
    \begin{table}[ht]
        \centering
        \begin{tabular}{|c|c|c|c|}
            \hline
             $(Y_{\psi(1)},Y_{\psi(2)})$ &$\p[(\psi)]{i}{2}$  & $\p[(\psi)]{j}{2}$ & $\p[(\psi)]{k}{2}$ \\\hline\hline
             $(0,0)$ &
             $\dfrac{\beta_i\alphaC_j p_i}{d_{(0,0)}}$ 
             & $\dfrac{\alphaC_i\beta_j p_j}{d_{(0,0)}}$
             & $\dfrac{\alphaC_i\alphaC_j p_k}{d_{(0,0)}}$ \\\hline
             $(0,1)$
             &$\dfrac{\beta_i\alpha_j p_i}{d_{(0,1)}}$  
             & $\dfrac{\alphaC_i\betaC_j p_j}{d_{(0,1)}}$ 
             & $\dfrac{\alphaC_i\alpha_j p_j}{d_{(0,1)}}$  \\\hline
             $(1,0)$ 
             & $\dfrac{\betaC_i\alphaC_j p_i}{d_{(1,0)}}$ 
             & $\dfrac{\alpha_i\beta_jp_j}{d_{(1,0)}}$ 
             & $\dfrac{\alpha_i\alphaC_jp_k}{d_{(1,0)}}$\\\hline
             $(1,1)$  
             &  $\dfrac{\betaC_i \alpha_jp_i}{d_{(1,1)}}$
             &  $\dfrac{\alpha_i\betaC_j p_j}{d_{(1,1)}}$
             & $\dfrac{\alpha_i\alpha_j p_k}{d_{(1,1)}}$\\\hline
        \end{tabular}
        \caption{The probabilities $\p[(\psi)]{i}{2}$, $\p[(\psi)]{j}{2}$, and $\p[(\psi)]{k}{2}$ (for all $k \notin \{i,j\}$) under different values of $Y_{\psi(1)}$ and $Y_{\psi(2)}$.}
        \label{second updates}
    \end{table}
    
    The probabilities for $\psi'$ can be obtained by swapping $i$ and $j$. Our result follows by comparing these values appropriately. 
\end{proof}
\begin{proof}[Proof of \Cref{order does not matter mid}]
    Since the first $t_1 - 1$ steps of $\psi$ and $\psi'$ are the same, $\p[(\psi)]{i}{t_1-1} = \p[(\psi')]{i}{t_1-1}$ for all $v_i \in V$. We can therefore just assume that our schedules start at $t_1$ and that $X = i$ has probability $\p[(\psi)]{i}{t_1-1}$. The result now follows from \Cref{two-step update} if $t_2 = t_1 +1$. Now, through a simple induction on $t_2 - t_1$, our claim follows: assume that the claim is true when $t_2 - t_1 = k$ for some $k$. If the difference is now $k+1$, then swap the positions of $\psi(t_1)$ and $\psi(t_2 - 1)$; followed by $\psi(t_2 - 1)$ and $\psi(t_2)$; and finally $\psi(t_1)$ and $\psi(t_2 - 1)$. The schedule so obtained is clearly $\psi'$.  
\end{proof}

\begin{proof}[Proof of \Cref{repeated searching of one node}] 
    By \Cref{order does not matter main thm}, we can assume that the first $Y_{\psi(t)} = 1$ for the first $a_i$ steps while for the rest ($b_i$ steps), $Y_{\psi(t)} = 1$. Using standard induction techniques on $a_i$ (using \Cref{update when searcher says yes} for the base case), we have (this equation was also derived as Claim 1 in \cite{cheng_scheduling_2021}):
    \[
        \p{j}{a_i} = 
        \begin{cases}
            \displaystyle\frac{\betaC_i^{a_i} p_i}{\betaC_i^{a_i} \cdot p_i + \alpha_i^{a_i} (1 - p_i)} \text{ if }j = i\\
            \displaystyle\frac{\alpha_i^{a_i} p_j}{\betaC_i^{a_i} p_i + \alpha_i^{a_i} (1 - p_i)} \text{ if }j \neq i
        \end{cases}
    \]
    Using similar arguments (with \Cref{update when searcher says no} as the base case and $\p{j}{a_i}$ as the base probability of $X = j$), we get:
    \[
        \p{j}{s} = \p{j}{a_i + b_i} =  
        \begin{cases}
            \displaystyle\frac{\beta_i^{b_i}\p{i}{a_i}}{\beta_i^{b_i}\p{i}{a_i} + \alphaC^{b_i}_i(1 - \p{i}{a_i})} \text{ if }j = i\\
            \displaystyle\frac{\alphaC_i^{b_i}\p{j}{a_i}}{\beta_i^{b_i}\p{i}{a_i} + \alphaC^{b_i}_i(1 - \p{i}{a_i})} \text{ if }j \neq i
        \end{cases}
    \]
    Plugging the value of $\p{j}{a_i}$ from the first equation into the second and simplifying gives us the required result.
\end{proof}
